A Norm Emergence Framework for Normative MAS -- Position Paper

Norm emergence is typically studied in the context of multiagent systems (MAS) where norms are implicit, and participating agents use simplistic decision-making mechanisms. These implicit norms are usually unconsciously shared and adopted through agent interaction. A norm is deemed to have emerged when a threshold or predetermined percentage of agents follow the "norm". Conversely, in normative MAS, norms are typically explicit and agents deliberately share norms through communication or are informed about norms by an authority, following which an agent decides whether to adopt the norm or not. The decision to adopt a norm by the agent can happen immediately after recognition or when an applicable situation arises. In this paper, we make the case that, similarly, a norm has emerged in a normative MAS when a percentage of agents adopt the norm. Furthermore, we posit that agents themselves can and should be involved in norm synthesis, and hence influence the norms governing the MAS, in line with Ostrom's eight principles. Consequently, we put forward a framework for the emergence of norms within a normative MAS, that allows participating agents to propose/request changes to the normative system, while special-purpose synthesizer agents formulate new norms or revisions in response to these requests. Synthesizers must collectively agree that the new norm or norm revision should proceed, and then finally be approved by an "Oracle". The normative system is then modified to incorporate the norm.

==> reviewers_comments.tex <==
\newenvironment{response}{\begin{quote}\color{blue}}{\end{quote}}

 \section*{Responses to Reviewers' Comments}

We would like to thank the reviewers for their detailed and insightful comments. Below we detail for each reviewer how we addressed their comments. The reviews are copied and we respond inline in blue. 



\section*{Editor's Comments} 
Insert if any

\begin{response}
Insert response
\end{response}

\section*{Reviewer \#1:} 
This paper proposes a novel framework for norm emergence in MAS, mixing a system where norms arise bottom-up from what agents are actually doing with the approach where new norms are explitictly entered into the system from an external source.

1. Relevance
The topic of this paper is interesting and relevant to COINE.

2. Significance
The topic of the paper is significant. As a position paper it proposes a new idea, but not the actual excecution yet, so it's significance lies more in the conceptial new ideas and discussion potential than in tangeable outcomes.

3. Novelty
The ideas proposed in this paper are novel

4. Quality of Presentation
The text of Figures 1 and 2 is very small, and very hard to read without a lot of zooming in. (Figure 2 became readable only at 300\% and comfortable to read at 400\%). I'd suggest changing them so they can actually be read at 100\% zoom. Some sections are quite long, and could have benefited from more subsectioning. In general, I feel the text could be shorter, as there is some repetition present.
\begin{response}
We have reconfigured figure 2 and made both diagrams more readable. 
We have rearranged the context section and split it into concepts to achieve some sub-sectioning.
\end{response}

%reconfigure figure 2. 
%consider vector graphics format for images. 

%have a look at context section and split into concepts. e

In general, I like this paper. However, I feel that as a position paper, it could have had more discussion on the choices presented (why things in the proposed system are as they are), and why the alternatives were discarded. As is, it is mostly a description of a plan.

\begin{response}
We have done some of this as much as possible within the page limit.
\end{response}

5. Potential for sparking discussion
This is a position paper, so it proposes a new type of framework, and has good potential for sparking discussion.


\section*{Reviewer \#2:} 
The paper describes a position of the authors with regards to the process of norm synthesis and emergence. The topic of the paper is very relevant to COINE and provides some interesting venues for discussion on the topic. It is interesting to see how the authors attempt to bring two fields of normative MAS (perscriptive vs. emergent) together, and try to solve the issue of engineering norms for multiagent systems.
The paper is well-written, although perhaps a bit verbose for a position paper (it could have been written with a more concise focus on the synthesis process, which is where most of the novalty lies).
\begin{response}
Insert response
\end{response}
%work on reducing and trimming

The paper definitely has the potential for sparking discussion. Some points from my side; I am wondering whether the synthesiser agents would need some form of filtering mechanism to cope with agents flooding the system with norm change requests. Second to that, I am wondering whether there is a need for the additional complexity of adding the Oracle, except for those cases where the MAS is included in a higher-level MAS. Wouldn't the synthesisers be able to decide (among each other) about other decisions regarding the norm inclusion/change?
\begin{response}
We inserted the need for filtering. Oracle? 
\end{response}

Other, more minor remarks:
In section 2.1, you advocate that agents would not have the capabilities of norm syntheses themselves (to which I fully agree), but do claim that agents can make proposals/requests to the synthesiser agents. What capabilities with regards to reasoning about the norms is required for the participating agents? Surely, not all agents can determine whether the results of their actions are due to some governing norms in the system. 
%should think along the lines
%challenge in the design on normative/practical reasoning agents - taking a decision that is norm compliant, inability to have a consciousness about it. actions triggered by beliefs, agents might not know that beliefs were included based on norms. Meta-reasoning missing where agents might not know why they are doing an action.
%maybe make clearer that agents are in a particular state and they are not happy
%NB: agents get feedback on actions from the environment, some of the feedback can contain normative information. 

How do you stop agents from 'blaming the system' for everything that does not work out to their liking (and thereby flooding the request system)?
%to think about how we might go about filtering requests 
%synthesisers have to decide which of these requests warrant action. where should the reflection process happen.
%participating agents must be required to make a decision about requests. naive agents may complain about everything, how can we make them 
%maybe include a system where they can complain and then get feedback where they can decide based on this feedback if to make an official complaint. agents need an opportunity to have a reasoning service. 
%think about an automated rejection process. 

In section 2.2, you further express the assumptions you make about the participating agents. I can agree to most, but am rather reluctant about "the agent is capable of perceiving a need for a norm change..". I believe most agents available today would be disqualified by that requirement/assumption.
%

Shouldn't synthesiser agents have a more pro-active role in the organisation? Since every participating agent is assigned a synthesiser, the synthesiser can observe what the agents are trying to perform, and identify potential norm changes. Moreover, I assume the synthesisers have some notion of the higher goals of the organisation.
%maybe mention that this can be an area for future work. 
%present both views as they are essentially just a discussion synthesiser


It is not entirely clear how much a synthesiser agent can actually perceive. Is the perception of all synthesisers complementary to each other; can they only perceive what their assigned agents can do?
%have a look back at this in hopes of making it clearer.


Very minor remark:
there appears to be some typo's in the second half of reference [10] and in reference [11] (underscores? and outlining).
%need to fix


\section*{Reviewer \#3:} 

>       The paper is highly relevant, providing a comprehensive framework for the emergence of norms. This is a significant contribution for the COINE conference. The paper is highly relevant for organizational studies or political science. The contribution is only of modest novelty, as many comparable attempts have been made in the past decade (e.g. Hollander and Wu (2011) The current state of normative agent-based systems; Frantz and Pigozzi (2018) Modelling Norm Dynamics in Multi-Agent Systems). However, it can be expected to stimulate significant discussions.
%have a read of these 2 and see how they relate
>       Some minor issues:
>       A) can you provide an explicit definition of the difference between MAS and normative MAS in the abstract?
\begin{response}
Thanks for your observation. This has now been included in the introduction rather than the abstract as suggested. 
Both papers present a review of state of the art in the research area and present a process model which doesn't actually account for insights in more current research nor specify a particular plan. [well the first one doesn't, second one is too long]
\end{response}
%COMMENTS - include in the introduction
%a decision has been made not to put it in the abstract but in the introduction. Normative MAS is a MAS that uses explicit norms and agents can decide whether to adopt or not. Sometimes norms are enforceable. 

>       B)I’m surprised that the authors found only example (AOCMAS) for decentralized norm emergence, as in the field of social simulation from Axelrod’s “evolutionary theory of norms” in the 1980s numerous examples can be found.

\begin{response}
It is possible that this was not as clear as it should be in the text but the reference here relates to decentralised online norm synthesis methods rather than norm emergence methods which we know there exists a vast amount of literature.
\end{response}
%COMMENTS - look to see how to make this more clearly and address this. 

>       C) Can you indicate potential fields of applications for the suggested framework? (e.g. in the case of political science suggestions for norm change that are detrimental for the overall system might appear quite regularly)
\begin{response}
We have chosen not to identify any specific domain at this point because we believe the framework is applicable to all types of MAS. The applicability to MAS is based on the fact that almost all MAS are likely to require changing norms throughout its lifetime. 
\end{response}

%COMMENTS - make it clear that the mechanism is applicable to all types of MAS. Maybe make it clearer that agents can't keep making changes.
